Watch Out for the Safety-Threatening Actors: Proactively Mitigating Safety Hazards

Despite the successful demonstration of autonomous vehicles (AVs), such as self-driving cars, ensuring AV safety remains a challenging task. Although some actors influence an AV's driving decisions more than others, current approaches pay equal attention to each actor on the road. An actor's influence on the AV's decision can be characterized in terms of its ability to decrease the number of safe navigational choices for the AV. In this work, we propose a safety threat indicator (STI) using counterfactual reasoning to estimate the importance of each actor on the road with respect to its influence on the AV's safety. We use this indicator to (i) characterize the existing real-world datasets to identify rare hazardous scenarios as well as the poor performance of existing controllers in such scenarios; and (ii) design an RL based safety mitigation controller to proactively mitigate the safety hazards those actors pose to the AV. Our approach reduces the accident rate for the state-of-the-art AV agent(s) in rare hazardous scenarios by more than 70%.

==> 01-intro-0517.tex <==
\section{Introduction}
\label{ml4ad:s:introduction}
Driving in a dynamic real-world environment among other actors is inherently a risky task. 
Each actor in the environment can significantly threaten safety by limiting the number of safe trajectories (as backup plans) and influencing the driving decisions of the autonomous vehicle (AV). 
In extreme cases, any of these actors can, willingly or unwillingly, thwart the AV's ability to complete the driving task safely.
Current approaches to developing self-driving agents, whether using an end-to-end agent (e.g., learning by cheating (LBC) agent~\cite{chen2019lbc}) or a multi-part agent composed of several deep learning models and heuristics (e.g., Apollo Baidu~\cite{apollo}), focus on reducing accidents or perception/planning/control errors, in the hopes that the agent can learn to identify important actors and create safety hazard mitigation plans with respect to those actors implicitly from data via training. 
However, it is unclear if the current approaches indeed learn to identify important actors (i.e., safety-threatening actors) and take actions that maximize safety.
Our evaluation of the state-of-the-art approaches (e.g., LBC) shows that autonomous agents have a high accident rate in rare hazardous driving scenarios. For example, of the thousand mutations of a cut in scenario, LBC agent collide in more than~{50\%} of the cases with the actor.
Thus, it is critical to develop techniques to (i) identify and quantify the threat posed by each actor in terms of their ability to create a safety hazard and (ii) proactively mitigate those threats by ensuring that safe navigational choices are always available AVs. 

\textbf{Our Approach.}
To achieve the goals above, we propose a reinforcement learning (RL)-based safety hazard mitigation controller (SMC) that uses causal and counterfactual reasoning to estimate the threat (referred to as safety threat indicator or \score) posed by an actor to the AV safety. 
The SMC execution is independent of the existing AV controller so that it does not interfere with the normal operation of the AV. 
This independent SMC approach (i) ensures low correlations between the ego actor's and the SMC's action and (ii) reduces the need to re-develop the ego actor for the additional mitigation actions.
Instead it continuously monitors the \score of each agent. It takes preventive and proactive actions such as braking, accelerating, or changing lanes to ensure that there are always safety plans (in this case, paths) available to the AV, thereby actively reducing the \score of each agent only when it is needed.  

\textbf{Estimating \score}.
Safety threat indicator (\score) characterizes the threat posed by an actor using causal and counterfactual reasoning. 
It is estimated with respect to the AV (hereafter referred to as the ego actor) for every other actor on the road (hereafter called the non-player character or NPC actor). It is directly proportional to a reduction in the number of safe navigational choices available to the ego actor in the presence of the NPC actor, which is semantically similar to an increase in the number of safe navigational choices in the absence of the actor (a counterfactual query). 
Our key insight behind the proposed approach is that decreasing safe navigational choices (backup options) makes the situation more constraining and prone to safety hazards, especially in driving scenarios where the allowed reaction time is significantly constraining.
We assert that such an indicator is akin to the reasoning used by humans to continuously be vigilant to safety-threatening actors. Humans avoid accidents by continuously reducing threats posed by these actors. 
The \score is normalized ([0,1]) to allow for ranking of both the NPC actors and the driving scenarios, and it depends on 
\begin{enumerate*}[label=(\roman*)]
	\item the environment (i.e., driving scenario) and 
	\item the uncertainty associated with determining the NPCs future trajectories.
\end{enumerate*}
The estimation\score requires reachability analysis for identifying available safe navigational choices~\cite{5509799}. 
Reachability analysis is computationally expensive, making it less applicable for real-time applications.
Thus we develop an interpretability-preserving neural network-based approximation technique for estimating the \score.

\textbf{Safety hazard mitigation.}
Based on our key insight above, we assert that proactively maintaining multiple safe navigational choices will create a safety blanket around the AV which will allow it to avoid safety hazards. 
This is because such a safety blanket allows AV to avoid getting into dangerous driving situations, to begin with, from which there is no point of return (e.g., accident) or significant impact to comfort (e.g., emergency braking).
It is more effective than reactive techniques (e.g., forward collision warning system~\cite{1336352}) as there might not be any other safe choice available to the AV at the time of the activation of reactive mitigation techniques.
We develop a reinforcement learning (RL)-based safety hazard mitigation controller (SMC) to proactively create safety bracket for AV to avoid high \score situations.
Mitigation actions such as braking and changing lanes could change the AV's dynamic drastically, so while these ac tions can reduce the \score, they trade off
passenger comforts and mission completion time for safety. Our SMC learns to balance these trade-offs via a RL based formalism with a multi-part reward functions that encodes
the benefits for reducing \score, the penalty for frequent mitigation activation, the benefits for normal driving in low \score situations to ensure mission completion, and
the benefits of maintaining comfort, as weighted sums. As a result, our SMC learns a balanced mitigation policy that proactively mitigates the scenarios that could lead to a
hazardous situation in the near future, while not affecting the normal driving when there is no such need. Finally, we train the SMC using Double-DQN algorithm [CITE DOUBLE
DQN] to action values overestimation to more effectively learn the mitigation policy.


\textbf{Contribution.}
\cref{fig:approach} conceptually describes the core idea of our paper. To the best of our knowledge, this is the first attempt at using counterfactual reasoning to characterize importance of each actor on the road with respect to safety of the AV which is then used to proactively mitigate the safety hazards by taking precautionary actions. \textbf{}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{resources/intro_figure.pdf}
    \caption{Safety threat indicator (\score) for a cut-in driving scenario with (a) safety mitigation controller (SMC) disabled (No-Op), and (b) SMC enabled (which decides to brake). 
    Each reachable grid (local goal location) represents a safe navigational path (from current location to goal location) while the path to unreachable grids are unsafe paths.
    The goal of the SMC is to maximize the number of available safe navigational choice so as to create the safety blanket around the AV.}
    \label{fig:approach}
\end{figure}
The main contributions of the paper are as follows:
\begin{enumerate}[noitemsep,nolistsep,leftmargin=*, label=(\roman*)]
	\item \textit{Safety importance metric formalization.} We propose a new indicator, safety-threatening indicator (or \score), to quantify the importance of each actor in the environment as well as the environment itself using causal and counterfactual reasoning. 
	
	\item \textit{Demonstration of \score on real world driving datasets.}
	We evaluated the proposed indicator on Argoverse dataset~\cite{Chang_2019_CVPR} to extract important actors and driving scenarios. For example, we find that {\it only} 1.9\% of the actors and 3.9\% of the driving scenarios have \score of \textgreater 0.9.
	
	
	
	\item \textit{NN-based \score evaluation for meeting realtime latency requirements.} 
	Estimating \score which meets latency deadlines is computationally difficult because estimating \score requires reachability analysis, which is computationally intractable. 
	We develop an interpretability-preserving neural network (NN)-based approximation techniques for estimating \score, which is 198\texttimes~faster when compared to the traditional planner-based \cite{5509799} \score estimation while achieving over $90\%$ accuracy on trained data. 
	
	\item \textit{Proactively mitigating safety hazards.}  We develop reinforcement learning-based safety mitigation controller (SMC) that proactively mitigate the safety hazards by taking precautionary actions (such as braking, accelerating or changing lanes) to reduce the \score score. 
	
	We demonstrate SMC (along with \score estimation) on Carla simulator and show that SMC enabled AV is able to reduce the number of accidents from 783 out 2000 driving scenarios to 286 out of 2000 driving scenarios. 
	
	
	
\end{enumerate}



==> checklist.tex <==
\section*{Checklist}


The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{refer to the abstract and intro.}
  \item Did you describe the limitations of your work?
    \answerYes{refer to conclusion and future works \label{ml4ad:s:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{They are included in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{They are specified in \cref{s:train_val} and as part of the supplemental material.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We reported standard errors for the NN reachability approximator inference latency by running multiple data points, refer to \cref{s:nn_accuracy}. We do not report standard errors on the NN reachability approximator precision/recall due to compute limitations. We do not report standard error on SMC evaluation as the simulation for each mutation run is deterministic.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We will list the hardware resources in the supplementary materials. %
}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited the \textit{Argoverse} dataset.}
  \item Did you mention the license of the assets?
    \answerYes{We mentioned it in the reference.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{They will be included as part of the supplementary material}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{The code and tools are licensed under the MIT License which is free-to-use. The dataset is licensed under the CC BY-NC-SA 4.0 which is free for non-commercial use.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

